MaD-Scientist: AI-based Scientist solving Convection-Diffusion-Reaction Equations Using Massive PINN-Based Prior Data

Large language models (LLMs), like ChatGPT, have shown that even trained with noisy prior data, they can generalize effectively to new tasks through in-context learning (ICL) and pre-training techniques. Motivated by this, we explore whether a similar approach can be applied to scientific foundation models (SFMs). Our methodology is structured as follows: (i) we collect low-cost physics-informed neural network (PINN)-based approximated prior data in the form of solutions to partial differential equations (PDEs) constructed through an arbitrary linear combination of mathematical dictionaries; (ii) we utilize Transformer architectures with self and cross-attention mechanisms to predict PDE solutions without knowledge of the governing equations in a zero-shot setting; (iii) we provide experimental evidence on the one-dimensional convection-diffusion-reaction equation, which demonstrate that pre-training remains robust even with approximated prior data, with only marginal impacts on test accuracy. Notably, this finding opens the path to pre-training SFMs with realistic, low-cost data instead of (or in conjunction with) numerical high-cost data. These results support the conjecture that SFMs can improve in a manner similar to LLMs, where fully cleaning the vast set of sentences crawled from the Internet is nearly impossible.

==> Algorithm/Algorithm_test.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm         %
%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[t]
\caption{Training a Transformer test}
\begin{algorithmic}[1]
\STATE \textbf{Input:} {A prior dataset $D \cup T$ drawn from prior $p(\mathcal{D})$}
\STATE \textbf{Output:} {A Transformer $\tilde{u}_{\theta}$ which can approximate the PPD}
\STATE Initialize the Transformer $\Tilde{u}_{\theta}$
\FOR{$i=1$ to $n$}
    \STATE Sample $\alpha \in \Omega$ and $D \cup T \subseteq \Tilde{r}(\alpha) \sim p(\mathcal{D})$
    \STATE ($D := \{(x_D^{(i)}, t_D^{(i)})\}_{i=1}^{N_D}$, $T := \{(x_T^{(j)}, t_T^{(j)})\}_{j=1}^{N_T}$)
    \STATE Compute loss $L_{\alpha} = \frac{1}{N_T} \sum_{j=1}^{N_T} \left\{ \Tilde{u}(x_T^{(j)}, t_T^{(j)}) - \Tilde{r}(x_T^{(j)}, t_T^{(j)})\right\}^2.$
    \STATE Update parameters $\theta$ with an Adam optimizer
\ENDFOR

\end{algorithmic}
\end{algorithm}


==> Table/Table4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
% Table 4             %
%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%% Table %%%%%%%%%%%%%
\begin{table*}[t]
\caption{$L_2$ absolute and relative errors for inferring 12 1D CDR equations. The model trained with $\beta, \nu, \rho_1, \rho_2, \rho_3 \in [1, 5] \cap \mathbb{Z}$ tests each equation with an integer parameters with range $1 \sim 5$. \textbf{c-d-r} represents convection-diffusion-reaction equation and $j$ has a range $1 \leq j \leq 3$.}
\vskip 0.15in
%\raggedright \textbf{PINN-Prior Average $L_2$ Absolute Error : \textnormal{0.1375}, $L_2$ Relative Error : \textnormal{0.2497}}
\begin{center}
\label{table:five_terms}
\begin{tabular}{lcccccc}
\toprule
\textbf{Class} & \textbf{System} & \textbf{Metric} & \parbox[c]{2.3cm}{\centering \textbf{Fisher \\ Reaction Term} \\ $(\rho_1 \neq 0)$} & \parbox[c]{2.3cm}{\centering \textbf{Allen-Cahn \\ Reaction Term} \\ $(\rho_2 \neq 0)$} & \parbox[c]{2.3cm}{\centering \textbf{Zeldovich \\ Reaction Term} \\ $(\rho_3 \neq 0)$} \\
\midrule


% Class Reaction
\multirow{6}{*}{$\exists \rho_j \neq 0$} & 

\multirow{2}{*}{\textbf{reaction}} & Abs. err & 0.1861 & 0.1510 & 0.2170\\ 
&& Rel. err & 0.2688 & 0.2492 & 0.3348\\ 

\cmidrule(lr){2-6}

&\textbf{reaction} & Abs. err & 0.0395 & 0.0219 & 0.0460\\  
&\textbf{-diffusion} & Rel. err & 0.0551 & 0.0308 & 0.0615\\ 

\cmidrule(lr){2-6}

& \multirow{2}{*}{\textbf{c-d-r}} & Abs. err & 0.0343 & 0.0144 & 0.0305\\ 
&& Rel. err & 0.0516 & 0.0202 & 0.0406\\ 

\cmidrule(lr){1-6}


% Class Non-Reaction
\multirow{6}{*}{$\forall \rho_j = 0$} & 

\multirow{2}{*}{\textbf{convection}} & Abs. err & \multicolumn{3}{c}{0.5027}\\ 
&& Rel. err & \multicolumn{3}{c}{0.4972}\\ 

\cmidrule(lr){2-6}

&\multirow{2}{*}{\textbf{diffusion}} & Abs. err & \multicolumn{3}{c}{0.1249}\\ 
&& Rel. err & \multicolumn{3}{c}{0.1573}\\ 

\cmidrule(lr){2-6}

&\textbf{convection} & Abs. err & \multicolumn{3}{c}{0.1861}\\ 
&\textbf{-diffusion} & Rel. err & \multicolumn{3}{c}{0.2688}\\ 


\bottomrule
\end{tabular}
\end{center}
\vskip -0.1in
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> format.tex <==
% This is the format and style instruction of ICLR2025.

\subsection{Style}

Papers to be submitted to ICLR 2025 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2025_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2025_conference.sty+ and \verb+iclr2025_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2025_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 10 pages for the main text of the initial submission, with unlimited additional pages for citations. 



\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.





\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.

\newpage


